SCAM! Transferring humans between images with Semantic Cross Attention Modulation

A large body of recent work targets semantically conditioned image generation. Most such methods focus on the narrower task of pose transfer and ignore the more challenging task of subject transfer that consists in not only transferring the pose but also the appearance and background. In this work, we introduce SCAM (Semantic Cross Attention Modulation), a system that encodes rich and diverse information in each semantic region of the image (including foreground and background), thus achieving precise generation with emphasis on fine details. This is enabled by the Semantic Attention Transformer Encoder that extracts multiple latent vectors for each semantic region, and the corresponding generator that exploits these multiple latents by using semantic cross attention modulation. It is trained only using a reconstruction setup, while subject transfer is performed at test time. Our analysis shows that our proposed architecture is successful at encoding the diversity of appearance in each semantic region. Extensive experiments on the iDesigner and CelebAMask-HD datasets show that SCAM outperforms SEAN and SPADE; moreover, it sets the new state of the art on subject transfer.

==> sections/exps_a_backup15Nov.tex <==
Here, we present the experimental results of \mname.

\todo{something that I miss here is to say why there are no more methods to compare against. if there are really really really really no other methods, then I propose to have a part where we explain why we cannot compare against some other existing methods (eg. SPADE).}

\noindent \textbf{Implementation details.}
We train all models for 50k steps, with batch size of 32 on 4 Nvidia V100 GPUs. \vic{For LIP and CelebAMask-HQ, we set $k{=}8$ latents per label of dim $d{=}256$; for iDesigner, $k{=}32$ for the background labels.}

\begin{comment}
\noindent \textbf{Implementation details.}
We train all models for 50k steps, with a batch size of 32 on 4 Nvidia V100 GPUs. We use AdamW~\cite{loshchilov2019decoupled} with learning rate of 0.0001 for the generator and the encoder, and 0.0004 for the discriminator with $\beta {=} (0.9,0.999)$. 
We set $k{=}8$ latents per label of dimension $d{=}256$.
Each time we use attention on a feature map or image, we first encode the image using 2D sinusoidal positional encodings, as attention acts on sets that do not include positional information. Note that adding positional encoding to the latents is not useful because latents can be seen as a set and not a sequence. Moreover, since the latents are going to be initialized from a learned vector, this learned vector can incorporate the positional information, if needed, and this information will propagate throughout the architecture.
\end{comment}

\noindent \textbf{Pose and style transfer protocol.} Given two images with their segmentation masks $(x_1,s_1){\in}(X,S)$ and $(x_1,s_2){\in}(X,S)$, we retrieve their style codes $ST_1 {=} E(x_1,s_1)$ and $ST_2 {=} E(x_2,s_2)$. We transfer the style from $x_2$ to the pose of $x_1$ by $x_{\text{pt}} {=} G(ST_2,s_1)$.
%
\textbf{Subject transfer.} To transfer the subject from $x_2$ to the context of $x_1$, we create $ST_{\text{mix}}$, where the style codes related to the background come from $ST_1$ and the remainder codes come from $ST_2$. Then, we retrieve $x_{\text{hr}} {=} G(ST_{\text{mix}},s_1)$.

\subsection{Datasets and Metrics}

% \noindent \textbf{LIP.} Look In Person~\cite{Gong_2017_CVPR} is extracted from COCO~\cite{lin2014microsoft} and contains images of people in different poses with 30k train and 10k test samples. 
% All images are annotated with segmentations for body parts (including clothes) using 20 labels. 
% LIP is challenging due to: (a) poor segmentation quality, (b) poor, variable image quality, (c) occlusions, and (d) containing images from body parts, instead of full-bodies.

\noindent \textbf{iDesigner}~\cite{idesigner} contains images from designer fashion shows, including 50 different designers with 50k train and 10k test samples. The images are of high-resolution, featuring full-bodies with background diversity. We annotate it in a semi-automatic way: 
we segment human parts with~\cite{li2019selfcorrection} and then merge the labels to end up with: face, body and background.

\noindent \textbf{CelebAMask-HQ}~\cite{lee2020maskgan} contains celebrity faces from CelebA-HQ ~\cite{karras2018progressive} with 28k train and 2k test images. The images are labelled with 19 semantic labels of high quality. %We use this dataset because it was the main dataset used by ~\cite{Zhu_2020} and we want to see if our architecture performs well on tasks other than subject transfer.

\noindent \textbf{Metrics.} We use PSNR, reconstruction FID (R-FID), and swap FID (S-FID). We compute R-FID between $X$ and $X_{\text{reco}} {=} \{G(E(x,s),s) | (x,s)\in (X,S)\}$, while we compute S-FID between $X$ and $X_{\text{swap}} {=} \{G(E(x,s_1),s_2) | (x,s_1)\in (X,S) \text{ and } s_2\in S,\text{ with } s1\neq s2\}$.


%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparison to the state of the art}
Here, we compare the proposed \nicolas{\mname to the state-of-the-art SEAN~\cite{Zhu_2020}, previous state of the art SPADE\cite{park2019semantic}. We also include a weaker baseline where we keep SEAN encoder that produce a single latent per semantic label and then split it into a set of smaller latents that we then feed to the SCAM Generator.Results are reported in Table~\ref{tab:quant-sota}.}


\begin{table}[t]
\begin{center}
		\begin{small}
		\resizebox{\linewidth}{!}{
\begin{tabular}{l|rrr|rrr}
\toprule
Method & \multicolumn{3}{c|}{\cellcolor{lavenderblue}{\textbf{iDesigner}}} & \multicolumn{3}{c}{\cellcolor{lavenderblue}{\textbf{CelebAMask-HQ}}} \\
& PSNR $\uparrow$ & R-FID $\downarrow$ & S-FID $\downarrow$ & PSNR $\uparrow$ & R-FID $\downarrow$ & S-FID $\downarrow$ \\
\midrule
SPADE~\cite{Zhu_2020} & 12.6   & 74.2  & 77.0 & 12.3 & 31.4 & 31.25 \\
SEAN~\cite{park2019semantic} & 14.5   & 48.7  & 54.2 & 15.6 & 28.3 & 37.2 \\
SCAM+SEAN enc~ & 17.6   & 33.2  & 38.4 & 17.7 & 28.0 & 31.9 \\
\mname & \textbf{21.1} & \textbf{15.1} & \textbf{30.3} & \textbf{22.8} & \textbf{17.9} & \textbf{27.4} \\
\bottomrule
\end{tabular}}
		\end{small}
	\end{center}
	\caption{\small{\textbf{Quantitative results} on iDesigner~\cite{idesigner} and CelebAMask-HQ~\cite{lee2020maskgan}. \todo{aren't there more methods to add here?} 
	\todo{S-PSNR maybe?} }}
\label{tab:quant-sota}
\end{table}

\noindent \textbf{Results on iDesigner} are shown in 
Table~\ref{tab:quant-sota}~(left). 
%
Overall, \mname outperforms SEAN and SPADE for all metrics. 
Specifically, for PSNR it outperforms SEAN by approximately +6.5dB, whereas it reaches 15.1  R-FID vs 48.7 for SEAN, i.e., +33. 
Both improvements are significant, which shows both that the reconstructed images with \mname better preserve the details of the initial images and that the representation power of \mname is higher than the one of SEAN. 
%
For S-FID, the difference is also notable, with SEAN reaching 54.2 vs 30.3 for \mname, i.e., +25. 
%
% Note that S-FID is significantly worse than R-FID; this is expected, as all methods are trained solely for reconstruction but not for swaps. 
% We argue that training on swaps would bring significant improvements to these results, but we leave this for future work.

\noindent \textbf{Results on CelebAMask-HQ} are shown in Table~\ref{tab:quant-sota}~(right), where we observe that \mname heavily outperforms \vic{all methods}. 
For instance, for PSNR, \mname SCAM outperforms SEAN by +7dB while having a 10 points lower R-FID than SEAN (17.9 vs 28.3), thus revealing its superiority for reconstruction. 
%
For swaps \todo{change name}, \mname highly outperforms SEAN by a S-FID decrease of almost 10 points (27.4 vs 37.2), clearly indicating that our method also is better at swapping over SEAN. 
Remarkably, these results are more interesting than the ones on iDesigner, as SEAN~\cite{Zhu_2020} is crafted to perform face swapping on this dataset.



%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ablations}

\input{tabs/ablation}

Here, we perform several ablations to validate the effectiveness of all components of \mname. 

\noindent \textbf{Ablations of SAT-Encoder and SCAM-Generator.}
Here, we examine the effectiveness of the the encoder and generator of \mname. 
For this, we modify either the SAT-Encoder or the SCAM-Generator with baseline versions and report the results on iDesigner in Table~\ref{tab:ablation-idesinger}, where the last row (vii) corresponds to our \mname. 
%
The first two rows correspond to our variants of our SAT-Encoder: (i) we use the same image at each SAT-Block without encoding it with convolution, and (ii) removing the SAT self-attention module.  
The results show that overall our SAT-Encoder (vii) outperforms both other variants (i,ii), e.g., -1-13 on R-FID and -0.2-6 on S-FID. The difference is particularly dominant for (i), probably because \todo{intuition why?}. 
%
In (iii,iv) we examine two versions of the SCAM-Generator (iii) without the SAT-Operation, (iv) without the Modulation operation (a,c in Section~\ref{subsub:scam}).  
In both cases, the proposed SCAM-Generator leads to better results; for instance, for (iii) +0.3db in PSNR, -2.1 in R-FID, and -0.4 in S-FID, indicating that both operations bring essential improvements. 

\noindent \textbf{Ablation of Losses.} 
Table~\ref{tab:ablation-idesinger}~(v,vi,vii) ablates the three $L_1,\mathcal{L}_{\text{Perc}},L_{\text{GAN}}$ losses used in \mname (Equation~\ref{eq:loss}) on iDesigner.  
%
Overall, using them all (vii) reaches the best results. 
Interenstingly, removing $\mathcal{L}_{\text{Perc}}$ (vi) results in the best PSNR point (22.3db) while having among the worst R-FID and S-FID (50.3, 113.5, respectively). 
This is expected as \todo{explanation?}. 

\noindent \textbf{Number of parameters (\#params).} 
A major benefit of \mname is the reduced \#params compared to SEAN, which are 4x fewer: \#params for \mname is 81M vs 214M for SEAN.  
This is because at each encoding layer, SEAN has a big FFN for each style code. By using a SCAM-Block instead, we greatly reduce the \#params while still achieving better performances.

\noindent \textbf{Number of $k$ latents per semantic label (\#kinlabel).} 
Using multiple latents per semantic label allows tuning the representative power in a \emph{semantic way}. Figure~\ref{fig:nb_latents} plots the FID scores (green for R-FID, orange for S-FID) over the \#kinlabel. 
We observe that the more \#kinlabel increases, the better the R-FID gets, \vic{highlighting that more latents lead to better reconstruction.} 
However, S-FID seems constant for all $k$ values, \vic{probably because we train \mname only for reconstruction and not for subject transfer.}

\begin{comment}

Here, we examine the effectiveness of SILA-E and SCAM-G.  
For this, we replace either the SILA-E or the SCAM-G of our method with the ones from SEAN and report the results in Table~\ref{tab:ablation-idesinger}. 
%
The first and last rows correspond to SEAN and our proposed \mname, respectively. 
The second row corresponds to the encoder from SEAN with our SCAM-G\footnote{Given that the SEAN encoder creates only one latent per semantic label, we partition the latent vector by splitting among its dimensions to obtain the desired number of latents.}. 
The results show that replacing the SEAN generator by SCAM-G brings significant improvements in all metrics, i.e., 5dB on PSNR, -50 on R-FID and -48 on S-FID. 
%
In (iii) we use the SILA-E by splitting the latent in 8 sublatents \todo{explain more}
%The fourth row corresponds to SILA-E with the SEAN generator.
Note, in this case the SEAN generator is essentially killing all attention mechanism from SILA-E, as it uses only one latent to attend to. Even in this case, \todo{fill in if we have good numbers; otherwise, remove}
%
In (iv) we report the case, where we use the same image at each SILA block without encoding it with convolution. 
Comparing to \mname in last row, we observe that by adding the convolution encoding of the input, we achieve a +2dB on PSNR, -6 on R-FID and -5 on S-FID. 
This shows that enabling the cross attention to attend at multiple resolutions is crucial. 
This is expected, as performing cross attention on the whole image, makes it difficult to capture low-resolution cues, which can be essential for reconstruction.
%
Moreover, we note that compared to the CelebAMask-HQ or iDesigner, SEAN performs poorly on LIP, due to its challenging nature (bad segmentations, several occlusions, high pose and background diversity, etc). 

\end{comment}




\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/attention_vis.png}
    \caption{\small{Last layer of \mname attention visualization on idesigner. We observe that (a) the model specializes some latents to reconstruct complex patterns (e.g., shirt, eyes, shoes), and (b) model is learning semantic information \emph{on its own} inside the semantic labels (e.g., people in the background). 
    \todo{1: increase font size of text} \todo{2: put (a), (b), (c), (d) below each image}}}
    \label{fig:attention_vis}
\end{figure}

\noindent \textbf{Visualization of the attention matrix.} 
Given that \mname uses multiple latents for every semantic region, here we examine which latent attends to which image region.
Specifically, in Figure~\ref{fig:attention_vis} we visualize the last \mname layer attention matrix; then, we assign a colour to every latent, and for each pixel we give it the colour of the latent with the highest attention value latent.
%
Overall, we observe that for each semantic region, the latents attend to different subregions, showing some unsupervised semantic knowledge. 
% In the first row (a), we see on the subject face label that we have some latents that specialize on eyes, mouth and hair attributes. We also see on the body segmentation label that some latents are learned for the different body parts, the dress and the shoes. labels that appear on
\vic{The first example (a) shows that even without specialized segmentation labels, \mname specializes some latents to reconstruct the complex face pattern (latents on eyes, mouth and hair) and others for the different body parts, dress and shoes. 
}
%
%On the second row (b), we now see that the background latent learns some latents to target the subject that haven't been labeled as humans and are in the background label. Even on this 'background humans', we see that SCAM assign different latents for each body part (hair and face latent for example). 
\vic{The second row displays an interesting case: 
\mname is capable of both detecting background humans (even if they are not labelled as human by the segmentation mask) and assigning different latents for their body parts (hair, face latent). This highlights the importance of background latents at modelling.}
\vic{Note that on both (a) and (b) the background labels manage to learn some general topology of the background such as walls, lighter zones, shadows; this suggests that \mname learns some semantic information \emph{on its own}.
}

\subsection{Qualitative results on iDesigner}
% similar structre as the quantitative results + comment on the images. In all cases you "need to" say: 
% (a) some comments about one or two examples (specifically pointing to particular examples) and  
% (b) something that holds "overall" 

Overall, we observe that the reconstruction quality of images with SCAM is superior to the ones from SEAN. This is mainly due to (a) having richer latents vectors thanks to the SILA encoder and (b) exploiting multiple latents enables a better generation process, and it helps gather a finer structure. \todo{for vicky to fix this part}

Here, we report subject and pose reconstruction and swap results on iDesigner.

\noindent \textbf{Subject Reconstruction.}
Figure~\ref{fig:reco_idesigner} displays the segmentation masks of the original images (first and second columns) and the reconstructed images when using SEAN~\todo{ref SEAN} and \mname (last two columns). 
%
We observe that \mname reconstructs more structure than SEAN both in the background and the human. 

For the \textit{background}, we observe that the curtains and window frame of the third row are well-reconstructed by \mname in contrast to SEAN reconstructions that includes colors but no other frame-cues. 
Similarly, unlike SEAN, \mname reconstructs a human-looking model on the background of the second row. Moreover, we observe traces of overfitting in SEAN, since it is reconstructing background people without them existing in the original image. 
%
Another interesting point  is the handling of the shadow of the models. Where SEAN totally fails to reconstruct the shadows, our model, SCAM, does manage to capture this information. We can see that overall, the backgrounds look like an average texture of the reference background.

For the \textit{subject}, \mname results in finer reconstructions compared to SEAN. 
For instance, in the person of the last row, \mname successfully retrieves some texture from the clothes, whereas SEAN results in a smoothed filling of the semantic region. 
%
\todo{add one more example from this figure}
%In this picture, we can also spot a problem with SEAN: latent contamination. We can see that the colour of the dress is changed and looks darker in some parts while having white parts. This is because we look around the subject, we have dark and white parts of the background. The SEAN encoder contaminates the latents thanks to the receptive field of the CNN. We can see that our model, SCAM, does not seem to have this kind of problems.
%
Finally, we observe that \mname manages to retrieve most of the face attributes, unlike SEAN that totally fails to retrieve faces. 

 


\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/reco_idesigner_2.png}
    \caption{\small{\textbf{Reconstruction} on the test set of iDesigner~\cite{idesigner}. \todo{1. remove title as it's duplicated with the caption.} \todo{2. see my several commnets in figure 6 and 7 and do the same here} }}
    \label{fig:reco_idesigner}
\end{figure}

\noindent \textbf{Pose transfer.}
Figure \ref{fig:pose_transfer_idesigner} illustrates pose transfer results for SEAN and \mname (last two columns), given the segmentation masks of the pose images (first two columns), and the style images (third column). 
Overall, the SEAN results are not visually pleasing, as the subjects are poorly reconstructed with vague, blurry details (last row), wrong colors (first row), and poor swaps (last row, due to averaging the background). 
In contrast, the results of \mname are perceptually better, as finer details are preserved (face in first row), the overall appearance is coherent (last row), and the background reconstruction with swaps is more detailed (last row). 
%
We also note that \mname leads to more realistic interaction of the subject with the floor than SEAN.


\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/pose_transfer_idesigner_2.png}
    \caption{\small{\textbf{Pose Transfer} on the test set of iDesigner~\cite{idesigner}. \todo{1. fix font size} \todo{2 to save space, you can remove the title of the figure, as it's written in the caption} 
    \todo{3. keep the subtitles only once per column}
    \todo{4. consider putting the subtitles below the images}
    \todo{5. check if you can also add (a), (b), ... next to the subtitle of each image } 
    }}
    \label{fig:pose_transfer_idesigner}
\end{figure}

\noindent \textbf{Subject transfer.} 
Figure~\ref{fig:human_replacement_idesigner} depicts the subject transfer results for SEAN and \mname (last two columns), given the segmentation masks of the pose and background images (first two columns), and the subject images (third column). 
%
\mname leads to superior subject (e.g., washed out colors in SEAN vs coherent structured clothing in \mname in the first row) and background (i.e., global background structure, positioning of people on the sides and their colours) reconstructions than SEAN. 
%
The second row depicts a typical failure case: although the results of \mname are better than SEAN, there are some artefacts appearing behind the subject. 
We hypothetize that training on the swapped images would solve this issue; but we leave this for future work.

\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/human_replacement_idesigner_2.png}
    \caption{\small{\textbf{Subject Transfer} on the test set of iDesigner~\cite{idesigner}. \todo{1. fix font size} \todo{2 to save space, you can remove the title of the figure, as it's written in the caption} 
    \todo{3. keep the subtitles only once per column}
    \todo{4. consider putting the subtitles below the images}
    \todo{5. check if you can also add (a), (b), ... next to the subtitle of each image } }}
    \label{fig:human_replacement_idesigner}
\end{figure}

%%%%%%%%%%%%%%%
\subsection{Qualitative results on CelebAMask-HQ}
For a fair comparison to SEAN~\cite{Zhu_2020} that focuses on CelebAMask-H for reconstruction and style transfer, we experiment \mname on CelebAMask-H.  
%Recall, \mname aims at subject transfer. 
Note, although \mname aims at subject transfer, our results both on reconstruction and style transfer look perceptually superior to the ones of SEAN, even for datasets and tasks that SEAN is intended.

\noindent \textbf{For reconstruction,} Figure~\ref{fig:reco_celeba} illustrates the results with SEAN and \mname (last two columns) for five masks and images (first two columns). 
Overall, \mname generates crisper and more realistic results than SEAN, in which the edges and contrast are weak. For instance, \mname leads to better preservation both of structure (e.g., fifth row, teeth reconstruction with great details) and of colors (e.g., third-fourth row, yellow patches in the eyes with SEAN); the latter is due to latent contamination that results from the average pooling mechanism of SEAN, which is  taking most of the eye's features from pixels outside the eye which are skin pixels. 

\noindent \textbf{For subject transfer,}  Figure~\ref{fig:style_transfer_celeba} displays SEAN and \mname outputs, where we note trends similar to reconstruction. 
The output of SEAN is smoothed out (both rows), it suffers from latent contamination (yellow eyes in second row, hair in first row), and it fails to capture fine details (both rows, the nose's shape wrongly comes from the mask). 
Remarkably, \mname produces sharp structures with emphasis on fine details (both rows, the noses come from the style image).


\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/reco_celebAHQ.png}
    \caption{\small{\textbf{Reconstruction} on CelebAMask-HQ\cite{lee2020maskgan} \todo{Same as all figures: 1. font size, 2. remove some examples that are not famous and you don't comment on, 3. add (a), (b), ...? 4. subtitles below images? }}}
    \label{fig:reco_celeba}
\end{figure}




\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/pose_transfer_CelebA.png}
    \caption{\small{\textbf{Style Transfer} on  CelebAMask-HQ\cite{lee2020maskgan}. \todo{Same as all figures: 1. font size, 2. remove some examples that are not famous and you don't comment on, 3. add (a), (b), ...? 4. subtitles below images? }
    }}
    \label{fig:style_transfer_celeba}
\end{figure}







==> sections/original_experiments.tex <==
\subsection{Datasets}

\paragraph{LIP} The Look In Person ~\cite{Gong_2017_CVPR} is a dataset that contains pictures of peoples in different poses. The images are then annotated, giving segmentation mask to the different parts of the body (clothes are also annotated). There are 20 different semantic labels. The dataset is extracted from Microsoft COCO ~\cite{lin2014microsoft}. It contains 30,462 samples in the train set and 10,000 samples for the test. This dataset is quite challenging because the quality of the segmentation masks are not very good. Also, the quality of the images is variable throughout the dataset. The dataset also suffers from a lot of occlusions. The images are not only from full-body persons, but there are pictures from different body parts.

\paragraph{iDesigner} The iDesigner ~\cite{idesigner} is a dataset containing images from designer fashion shows. The dataset was proposed to classify images from 50 different designers. This dataset is high resolution with good image quality. This dataset contains 50,000 samples in the train set and 10,000 samples in the test set. Most of the pictures features full-body pictures, with some background diversity. We annotate ourselves the dataset using a pretrained segmentation network. We use the human parser network ~\cite{li2019selfcorrection} that segment human parts between 20 semantic labels. This semantic labels are the same that are used in LIP.

\paragraph{CelebAMask-HQ} The CelebAMAsk-HQ ~\cite{lee2020maskgan} is a dataset of celebrities faces. It contains 28,000 train images and 2,000 test images. The images are taken from CelebA-HQ ~\cite{karras2018progressive}, which curates the best celebrities faces pictures according to image quality. The images are then manually labelled according to 19 different semantic labels. The semantic labels from this dataset are of very high quality. We use this dataset because it was the main dataset used by ~\cite{Zhu_2020} and we want to see if our architecture performs well on tasks other than subject transfer.

\subsection{Metrics}
The metrics used in this work are the following: PSNR and FID. The two metrics derived from FID that we are going to use are reconstruction FID (R-FID) and swap FID (S-FID). For the reconstruction FID, we compute the FID between $X$ and $X_{reco} = \{G(E(x,s),s) | (x,s)\in (X,S)\}$. Then for the swap FID, we compute the FID between $X$ and $X_{swap} = \{G(E(x,s_1),s_2) | (x,s_1)\in (X,S) \text{ and } s_2\in S,\text{ with } s1\neq s2\}$.

\subsection{Experimental details}
We train all our models for 100,000 steps, with a batch size of 32 on 8 Nvidia V100 GPUs. We use the AdamW optimizer \cite{loshchilov2019decoupled} with a learning rate of 0.0001 for the generator and encoder and 0.0004 for the discriminator. For all networks we use $\beta = (0,0.9)$. Similar to SPADE \cite{park2019semantic} and SEAN \cite{Zhu_2020}, we use spectral normalization in both the generator and the discriminator. Finally, we use Synced BatchNorm to speed up the training. For all semantic labels, we have 8 latents of dimension 64.

To perform pose transfer (or style transfer), we have $(x_1,s_1)\in(X,S)$ and $(x_1,s_2)\in(X,S)$ two images and their segmentation masks, respectively. We then retrieve the style codes $ST_1 = E(x_1,s_1)$ and $ST_2 = E(x_2,s_2)$. If we want to transfer the style from $x_2$ to the pose of $x_1$, we can then do $x_{pt} = G(ST_2,s_1)$.

Similarly, to do subject transfer, if we want to transfer the subject from $X_2$ to the context of $X_1$, we create $ST_{mix}$ where we take the style codes related to the background in $ST_1$ and the rest style codes are taken from $ST_2$. Then, we can retrieve $x_{hr} = G(ST_{mix},s_1)$.

\subsection{Quantitative Results}
Here, we compare the proposed SCAM to the state-of-the-art SEAN~\cite{Zhu_2020}. 
Table~\ref{tab:quant-idesigner} reports the results for the PSNR, Reconstruction FID and Swap FID metrics. 
\paragraph{Results on iDesigner}
% add table and just comment on the results
We are first going to look at the results on iDesigner, which features full body persons.
%
We observe that overall, SCAM outperforms SEAN for all metrics. 
Specifically, for PSNR (higher is better) it outperforms SEAN by approximately +4dB, whereas it reaches 13.3  Reconstruction FID (lower is better) vs 20.43 for SEAN, i.e., +7. Both these improvements are significant, which shows that the reconstructed images with SCAM better preserve the details of the initial images and that the representation power of SCAM is higher than the one of SEAN. 
%
For Swap FID (lower is better), the performance difference is even more notable, with SEAN reaching 30.62 vs 22.24 for SCAM, i.e., +8. 
%
%Note that since both SCAM and SEAN are trained only for reconstruction, the FID for swaps is significantly worse than the one for reconstruction. 
Note that FID for swaps is significantly worse than FID for reconstruction; this is expected, as both SCAM and SEAN are trained solely for reconstruction but not for swaps. 
We argue that training on swaps would bring significant improvements to these results, but we leave this for future work.

% rich 
% representation 
% robustness 
% accross all metrics 
% outperforms, reaches, 
% increase, boost, improves 
% decreases , is inferior/superior
% leads to, results in + ing
% argue/hypothetize/estimate/believe
% We observe 
% therefore, hence 
\begin{longtable}[c]{c|c|c|c|}

\cline{2-4}
                                                   & \cellcolor[HTML]{9B9B9B}PSNR $\uparrow$ & \cellcolor[HTML]{9B9B9B}R-FID $\downarrow$ & \cellcolor[HTML]{9B9B9B}S-FID $\downarrow$ \\ \hline
\endhead
%
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}SEAN ~\cite{Zhu_2020}} & 15.49                        & 20.43                                      & 30.62                            \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}SCAM} & \textbf{19.53}               & \textbf{13.3}                              & \textbf{22.24}                   \\ \hline

\caption{Quantitative results on iDesigner~\cite{idesigner}}

\label{tab:quant-idesigner}\\
\end{longtable}



\paragraph{Results on CelebAMask-HQ}
% add table and just comment on the results
We are now going to look at results on the CelebAMask-HQ~\cite{lee2020maskgan} dataset. This is interesting to look at, since SEAN~\cite{Zhu_2020} was crafted to perform face swapping on this dataset.
%
We can see in Table \ref{tab:quant-celeba} that our method, SCAM, heavily outperforms SEAN in all metrics.
%
Looking at PSNR (higher is better) SCAM outperforms SEAN by approximately +4.5dB. Similarly, SCAM has a 7 points lower reconstruction FID (lower is better) than SEAN (18.99 vs 27.51). This shows that even if SEAN was tailored to work with CelebAMAsk-HQ dataset, we highly outperform it on the reconstruction task. As in iDesigner, for both methods the FID value is higher for the swap then for the reconstruction task, which is, as we stated, expected since we are training on a reconstruction task. However, SCAM highly outperforms SEAN by a swap FID decrease of almost 10 points (23.51 for SCAM VS 33.41 for SEAN), proving that our method also is better at swapping over SEAN.
\begin{longtable}[c]{c|c|c|c|}
\cline{2-4}
                                                   & \cellcolor[HTML]{9B9B9B}PSNR $\uparrow$ & \cellcolor[HTML]{9B9B9B}R-FID $\downarrow$ & \cellcolor[HTML]{9B9B9B}S-FID $\downarrow$ \\ \hline
\endhead
%
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}SEAN~\cite{Zhu_2020}} & 15.60                        & 27.51                                      & 33.41                            \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}SCAM} & \textbf{20.22}               & \textbf{18.99}                             & \textbf{23.51}                   \\ \hline
\caption{Quantitative results on CelebAMask-HQ~\cite{lee2020maskgan}.}
\label{tab:quant-celeba}\\
\end{longtable}

\paragraph{Ablation on LIP}
% add table and just comment on the results
Now, we are going to see how does SCAM perform on the more challenging LIP dataset. We are going to do an ablation study on this dataset. To do this, we set up some experiments. First we have SCAM + SEAN encoder, where we use the SEAN encoder to create the latents. However, SEAN is capable of creating only one latent per semantic label. Indeed, the latents are created by average pooling a CNN feature map. To solve this, we decide to partition the latent vector by splitting among the dimension of the latent vector to obtain the number of latents that we want. Then we have SCAM + SILA noconv where we use the SILA encoder, except that we use the same image at each SILA block. We do not encode it with convolution. Finally, we have SCAM + SILA which is our main model.

Table \ref{tab:ablation-lip} shows the results of the ablation. First, we can see that only changing the generator, we outperform SEAN by a large margin. It is to be noted that in this dataset, SEAN performs poorly compared to what it can achieve on CelebAMask-HQ or iDesigner. This is mainly due to the fact that LIP is a harder dataset with bad segmentations, lots of occlusions, a lot of diversity in poses, background, etc... While changing the generator manage to outperform SEAN by 5dB on PSNR, -50 FID points on reconstruction and -48 FID points on FID, we can see that the SILA encoder brings its own improvement. While only having the semantically masked cross attention does not bring a big improvement on its own (0.5dB on PSNR over using the SEAN encoder, -6 FID points on reconstruction and 1 on swapping) we see that by adding the convolutions encoding of the input, we achieve a +2dB increase on PSNR, -6 on reconstruction FID and -5 on swapping FID. This shows that enabling the cross attention to attend at multiple resolutions is very important for it to work well. Indeed, when we perform cross attention on the whole image, it is hard for it to capture low resolution information, which can be very important to capture the information of the image and be able to reconstruct it. This ablation study shows that both the generator and the encoder architecture are meaningful improvements over SEAN.


\begin{longtable}[c]{c|c|c|c|}
\cline{2-4}
                                                          & \cellcolor[HTML]{9B9B9B}PSNR $\uparrow$ & \cellcolor[HTML]{9B9B9B}R-FID $\downarrow$ & \cellcolor[HTML]{9B9B9B}S-FID $\downarrow$ \\ \hline
\endhead
%
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}SEAN ~\cite{Zhu_2020}}                  & 11.11 & 82.27 & 87.31 \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}SCAM + SEAN enc}   & 16.13 & 30.28 & 39.16 \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}SCAM + SILA noconv} & 16.65 & 24.53 & 37.57 \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}SCAM + SILA} & \textbf{18.61}               & \textbf{18.20}                             & \textbf{32.87}                   \\ \hline
\caption{Quantitative results on LIP~\cite{Gong_2017_CVPR}.}
\label{tab:ablation-lip}\\
\end{longtable}

\paragraph{Number of parameters} One of the benefits of our architecture is the reduced number of parameters. We see in Table \ref{tab:nb_parameters} that our method SCAM has 4x times fewer parameters as SEAN. This is due to the fact that at each layer, SEAN has a big Feed Forward network to map each style code. By removing this constraint and replacing it with our SILA block and the Semantically Cross Attention Block, that both share the mapping networks between latents, we manage to greatly reduce the number of parameters used in the model and still achieving better performances.
\begin{longtable}[c]{c|c|}
\cline{2-2}
                                                   & \cellcolor[HTML]{9B9B9B}Number of parameters \\ \hline
\endhead
%
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}SEAN~\cite{Zhu_2020}} & 214M                                         \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}SCAM} & \textbf{65M}                                 \\ \hline
\caption{Number of parameters of the different generator architectures }
\label{tab:nb_parameters}\\
\end{longtable}


\subsection{Qualitative Results}
% similar structre as the quantitative results + comment on the images. In all cases you "need to" say: 
% (a) some comments about one or two examples (specifically pointing to particular examples) and  
% (b) something that holds "overall" 
Overall, we observe that the reconstruction quality of images with SCAM is superior to the ones from SEAN. This is mainly due to (a) having richer latents vectors thanks to the SILA encoder and (b) exploiting multiple latents enables a better generation process, and it helps gather a finer structure.

\paragraph{Results on iDesigner}
On the iDesigner dataset, we can observe that on the reconstruction task, our model performs better background and subject reconstruction than SEAN. We can, for example, look at the 3rd row of Figure \ref{fig:reco_idesigner}. We see that our model, SCAM reconstructs a lot more structure in the background such as curtains or the window frame, whereas SEAN fails to reconstruct the background. In SEAN, we can see the colour of the curtains, but we do not see anything about the windows, or something that looks like a curtain. Similarly, if we look at the background of the second row, we can see that our method manages to reconstruct a human looking model in the background whereas SEAN reconstructs a floating blob. We can also see that SEAN might have overfitted, since it is reconstructing people on the side of the background in places that there is none. SCAM puts the people on the side of the picture in the right place. Another interesting point  is the handling of the shadow of the models. Where SEAN totally fails to reconstruct the shadows, our model, SCAM, does manage to capture this information. We can see that overall, the backgrounds look like an average texture of the reference background.

Respective to the reconstruction of the subject, we can see that SCAM gives a much better reconstruction. Where SEAN totally fails to retrieve the faces, SCAM manages to retrieve most of the attributes of the faces. Similarly, if we look at the 4th row, SCAM manages to retrieve some texture from the clothes, where SEAN gives a smoothed filling of the semantic region. In this picture, we can also spot a problem with SEAN: latent contamination. We can see that the colour of the dress is changed and looks darker in some parts while having white parts. This is because we look around the subject, we have dark and white parts of the background. The SEAN encoder contaminates the latents thanks to the receptive field of the CNN. We can see that our model, SCAM, does not seem to have this kind of problems.

\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/reco_idesigner_2.png}
    \caption{Reconstruction on the iDesigner~\cite{idesigner} dataset}
    \label{fig:reco_idesigner}
\end{figure}

Regarding Pose Transfer, we can see some results in Figure \ref{fig:pose_transfer_idesigner}. We can see that the results on SEAN are not very satisfying. If we look at the first row, we can see that the subject seems to be badly reconstructed. Especially, the colours of the subject are wrong. Again, this is due to the latent contamination problem in SEAN that we can observe in the reconstruction. The dress colours are much better in SCAM. Similarly, we can see that the subject has finer details, especially looking at the face. If we look at the second row, we can see that the background reconstruction with swaps is better with our method. Similar to the reconstruction task, SEAN seems to be generating an averaged background where we have a more successful background swapping. The subject interaction with the ground seems to be more realistic. Overall, the subject has also a much better reconstruction.


\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/pose_transfer_idesigner_2.png}
    \caption{Pose Transfer on the iDesigner~\cite{idesigner} dataset}
    \label{fig:pose_transfer_idesigner}
\end{figure}

If now we perform subject transfer, we see similar results to the ones with pose transfer. If we look at Figure \ref{fig:human_replacement_idesigner}, in the first row, we can see that  the subject has a better reconstruction, especially from the colours that are washed out in SEAN. The dress has also more coherent structure. The background  is again of a superior quality with SCAM. We see that in the background from SCAM, the global structure of the background is better preserved. Especially the positioning of the persons on the sides (and their colours). On the second row, although the results of SCAM are better than SEAN, we can see some artefacts appearing behind the subject. We hope to solve this issue by training on the swapped image in the future

\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/human_replacement_idesigner_2.png}
    \caption{Subject Transfer on the iDesigner~\cite{idesigner} dataset}
    \label{fig:human_replacement_idesigner}
\end{figure}


\paragraph{Results on CelebAMask-HQ}
As we stated before, we want to get results on CelebAMask-HQ, because SEAN~\cite{Zhu_2020} has focused on this dataset to perform style transfer. We want to show that although we tried to achieve subject transfer with our architecture, we manage to have good results on the same task as SEAN. For the reconstruction task, we can see that overall, our method, SCAM, generates much crisper results. We can see that with SEAN, the output image seems to be very soft. We can, for example, have a look at the 5th row, where our output seems to be more realistic. The colours are better preserved, and the overall structure is better. If we focus on the teeth, for example, we are able to reconstruct them with greater details. Similarly, that on iDesigner, we can see the latent contamination problem. This is notable for the second and fourth row, where we see for example some yellow in the eyes. This is due to the fact that the semantic region of the eyes is very small. However, if we consider the neighbouring pixels impacted by the receptive field of the CNN, we understand what is happening: The average pooling mechanism is actually taking most of the eye's features from pixels outside the eye which are in fact skin pixels. 
\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/reco_celebAHQ.png}
    \caption{Reconstruction on the CelebAMask-HQ\cite{lee2020maskgan} dataset}
    \label{fig:reco_celeba}
\end{figure}

Now, if we look at the swaps, we can see again that our method seems to produce crisper images. We can see that the output from SEAN is very smoothed out. We again see the latent contamination problem with SEAN in the second row, producing yellow eyes. We can also notice that SEAN struggles with the hair on the image in the first row. We can also notice that in both images, for SCAM the shape of the nose is very similar to the one in the style image, whereas SEAN seems to be only relying on the segmentation mask for the shape of the nose. We can say with confidence that our results look better on CelebAMaskHQ, and therefore our method successfully improves the results on the dataset that SEAN was supposed to work well. Other results can be seen in Figure \ref{fig:sean_celeba_swap_app} and \ref{fig:scam_celeba_swap_app}


\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/pose_transfer_CelebA.png}
    \caption{Style Transfer on the  CelebAMask-HQ\cite{lee2020maskgan} dataset}
    \label{fig:style_transfer_celeba}
\end{figure}


\paragraph{Visualization of the attention matrix}

Since we are using multiple latents for every semantic region, we can look what latent attends to which image region. We can see such visualization in Figure \ref{fig:attention_vis}. To do this, we visualize the last SCAM layer attention matrix. We then assign a colour to every latent, and for each pixel we give it the colour of the latent with the highest attention value latent. We can see that for each semantic region, the latents attend to different subregions. If we look at the last row, it is interesting to notice that, for example, the model seems to have used some latents to reconstruct the complex pattern on the shirt of the guy. We can also see that the model has specialized some latests on the face to reconstruct eyes, a mouth and the nose. Finally, it is interesting to notice that if we look at the smartphones regions, they seem to be both attended by the same dark green latent. This shows that the system has learned some kind of semantic information on its own.

\begin{figure} 
    \centering
    \includegraphics[width=\columnwidth]{images/attention_vis.png}
    \caption{Last layer of SCAM attention visualization on LIP}
    \label{fig:attention_vis}
\end{figure}


==> sections/original_intro.tex <==
%motivation 
The motivation behind this work is to be able to perform subject transfer between two images. We have one target subject and one source subject. The idea is that the source subject should replace the target subject in the target image seamlessly. The target image should keep the same background, the same interactions between objects and subject and occlusions should be dealt with. This lead us to look into semantic editing. Semantic editing consist in controlling the output of a generative network by a segmentation mask. It looks like a good solution for subject transfer, since we can both deal with the pose using semantic masks and the style of each semantic region. Semantic Editing techniques are useful because they can allow for fine editing of an existing picture.
\begin{figure}[t]
    \centering
    % link to the figure: https://drive.google.com/file/d/16iHvAEAgobre043x6pG2Gv_8zjLxAC_0/view?usp=sharing
    \includegraphics[width=\columnwidth]{images/teaserv2.pdf}
    \caption{Overview of our method for subject transfer. We first encode the desired subject we want to transfer with the Semantic Image to Latent Attention (SILA) encoder and get the subject latent codes. Then, we encode the background and the semantic mask for the pose and background reference. Finally, the Semantic Cross Attention Modulation (SCAM) generator will synthesize an image where the subject is transferred with the desired background and pose.}
    \label{fig:my_label}
\end{figure}

% applications
This problem is interesting because it could allow for multiple applications. It could be, for example, used to replace a stuntman by the main actor in an action movie, alleviating the constraint of finding a look-alike stuntman, and give more freedom to the filmmakers. Similarly, it could allow finishing a movie when an actor is indisposed. Since our technique allows for style editing, this could also allow for virtual try-on in any situation. 

Finally, privacy is starting to become  a big concern in the Machine Learning community. This technique could allow replacing real people in datasets that involve full-body persons.

% challenges
The task of subject replacement is quite challenging for multiple reasons. First, on the contrary of faces, buildings, or landscape, human bodies are malleable. They also have a lot of morphological diversity, making it harder to model. The task itself is hard since on the contrary of pose transfer, where we change the subject pose in the same picture, or of style transfer, where we keep the pose fixed and try to change the styling of the subject, here, we want to both change the pose and the style/identity of the subject in the picture. This makes it a lot harder to accomplish. It is to be noted that if we manage to do subject replacement, we can do both pose transfer and style transfer on human subjects for free.

% % goodies of editing 
% The semantic editing of images is also fascinating because it allows us to control finer regions inside an existing image. GAN Inversion techniques have tried to edit existing images with a pretrained GAN, but it is quite hard to have a good reconstruction of existing images. It's also challenging and can be resource demanding to find the right directions in the GAN latent space to perform the desired modification. It is also very hard to edit the pose with the same control that we have with semantic masks. Semantic masks allow to 'paint' what we want to get in the output image, like it was showcased by works such as SPADE \cite{park2019semantic}. The semantic mask is rich in information on the pose of the subject and modifying the latent space of the underlying GAN, it is possible to modify the style of the image.  These techniques can be very useful for image editing software.


PISE \cite{zhang2021pise} proposes to handle the pose transfer task using a SEAN~\cite{Zhu_2020} like network. This, however, suffers from the drawbacks of SEAN that does not allow handling complex backgrounds. Everybody Dance Now~\cite{chan2019everybody} does manage to reconstruct more complex backgrounds, but it needs to overfit a network to a very long training videos (more than 30 min). It then controls the learned subject with a pose skeleton. This is quite problematic since we need to train a GAN for every subject we want to transfer pose to. Also, we cannot change the background for a given subject and collecting all this data is unpractical. Training a GAN for each subject reveals impossible to use for real-life usage. Few Shots Video-to-Video Synthesis \cite{wang2018fewshotvid2vid} solves this issue with a hyper-network that tune the weights of the generator, but this is hard to train, and we see that in practice, it works with very simple backgrounds. None of this works perform both pose and subject transfer simultaneously.


Regarding semantic editing, SPADE \cite{park2019semantic} was the first work to give finer control to a user using semantic masks. However, SPADE suffers from not being able to control each region style independently. This was fixed by SEAN\cite{Zhu_2020}, where every semantic region gets its own style code. However, we observed that in practice, when the semantic region is not very detailed (for example, a background that can contain multiple objects, but has a single label), SEAN tends to fail to give a good output. 


In this work, we build a semantic editing system that can account for the challenges that are relevant to subject transfer. With our system, we find more carefully crafted latent variables for each semantic region, allowing for finer details in the reconstructed output. We also add more than one latent per semantic region, allowing for more complex information to be processed. Doing this, we outperform SEAN on the semantic editing task and allow us to perform subject transfer without having to train one network per subject. We are able to generate more complex scenes, where the background is not necessarily uniform.


To achieve this, we propose several modifications to SEAN. We first introduce Semantic Cross Attention (SCA), a mechanism to perform attention between a set of latents that are each linked to a semantic region and an image feature map, constraining the attention such as the latents can only attend the regions on the image feature map that correspond to the relevant feature map. Building around this, we introduce the Semantic Image to Latent Attention (SILA) and build an encoder around this block. This is what allows us to capture richer information in the encoding process. Finally, we modify the generator, to modulate the feature maps using the learned latents using Semantic Cross Attention Modulation (SCAM) to allow every pixel to attend to the semantically meaningful latents.

==> sections/original_method.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{images/encoder_generator_arch.png}
     \caption{First, the image is encoded using The Semantic Image to Latent Attention (SILA) encoder. SILA allows the latent to retrieve information from an image or an image feature map, restricted by a semantic mask. The SILA encoder allows the latents to retrieve information from an image, exploiting both the raw image and the convolution feature maps. Once the image is encoded, the latents are fed to the Semantic Cross Attention Modulation (SCAM) generator. At each resolution, the SCAM block update both the latents and the feature maps. It also progressively grows the output RGB image. The SCAM Generator captures top-down and bottom-up interactions with a semantic constraint, allowing to easily alter the desired regions thanks to the latents that are dedicated to a given region.}
    \label{fig:arch}
\end{figure*}



%In this work, our goal is to perform subject transfer while improving the semantic editing. Subject transfer is more challenging than pose transfer. Unlike pose transfer that focuses solely on the subject pose, subject transfer requires changing both the \emph{subject pose} but also the \emph{general context} in which the subject is situated.
In this work, our goal is to perform subject transfer while improving the semantic editing. Unlike \vic{the standard} pose transfer \todo{Ref} that focuses \emph{solely} on the subject pose,\textbf{ subject transfer} requires changing both the \emph{subject pose} but also the \emph{general context} in which the subject is situated\vic{; hence, it is more challenging than pose transfer.}
%
To this end, we introduce a method that improves upon the recently proposed SEAN~\cite{Zhu_2020}. SEAN proposes to perform semantic editing by assigning one style vector per semantic region, modulating the generated feature maps by the corresponding semantic region.
However, we observe that SEAN has two main shortcomings. 

\textit{First}, it performs poorly when it reconstructs inputs where the semantic mask is not refined enough. Such an indicative example is the background reconstruction. If we use two segmentation labels, one for the background and one for the subject, the resulting background semantic information is poor.
%
Using a single style vector for the background does not allow SEAN to capture the diversity of backgrounds, and instead, tends to generate blurred and generic backgrounds.
%
To address this, we build upon the GANsformer~\cite{hudson2021generative} and introduce a novel \textbf{S}emantic \textbf{C}ross \textbf{A}ttention \textbf{M}odulation (coined \textbf{SCAM}) that allows the generator to capture richer information.
%
Indeed, the Duplex Attention mechanism of the GANsformer allows the generator to capture semantic meaningful information in an unsupervised way.
%
Therefore, SCAM exploits this property and improves our generator in these challenging situations. 

\textit{Second}, the number of parameters in SEAN is very high, and it explodes when adding semantic labels.
%
Instead, as the number of semantic labels increases, the proposed SCAM requires much fewer parameters than SEAN, thus allowing for a lighter model.

The second contribution of our work is a way to encode semantically meaningful latent variables.
To obtain the style vectors, the commonly used SEAN uses a CNN to extract a representation and then performs global average pooling according to the semantic mask of the encoded image
%
This approach has three main shortcomings.
\textit{First}, we can only obtain one style vector per semantic mask. Having this monolitical style vector can limit the representation power, in particular for coarse semantic regions. GANsformer \cite{hudson2021generative} shows that having multiple style vectors can be beneficial to capture finer semantic representations.
%
\textit{Secondly} and more importantly, all the spatial information contained in the feature map is just averaged.
%
This is suitable for cases where the semantic label is very specialized, such as `eyes in a face'; however, when it comes to coarser labels (e.g., background), it fails to capture any meaningful information.
%
Following the work of Perceiver~\cite{jaegle2021perceiver}, we propose the \textbf{S}emantic \textbf{I}mage to \textbf{L}atent \textbf{A}ttention (\textbf{SILA}),  an encoder that relies on cross attention.
Given a set of latents, the main idea is to let the encoder decide (a) which information to gather in the image, and (b) for which latent.
% 
The encoder attention is constrained, i.e., it can only attend to the image region with the segmentation label that the latent is attributed to.
%
This architectural change also allows to have multiple latents for each segmentation label. 
%
It is very flexible and straightforward to give more representation power to certain segmentation labels by giving more latents related to the given segmentation labels.

\textit{Thirdly}, the last shortcoming is latent contamination. 
%
Since the receptive field of the CNN increase with its number of layers, the global average pooling operation contaminate the style codes with information from the neighbouring semantic regions. The problem is that the style code quality is going to be degraded and the disentanglement property between style codes can be lost.

The 2 methods cited above rely on a trick performed on the attention matrix called Semantic Cross Attention. The idea is that when using cross attention, the attention mechanism is restricted such that each latent can see only information from the respective semantic region. It is done with a masking of the attention matrix according to the segmentation masks. This allows to hard code what pixel can each latent see (Or in the case of SCAM what latents can each pixel see).

To summarize, we propose 3 new methods:

\begin{enumerate}
    \item A masking technique in cross attention, the Semantically Masked Attention.
    \item A way to encode semantically meaningful latent variables, SILA. 
    \item A way to modulate a GAN's generator feature map according to a segmentation map, SCAM.
\end{enumerate}

\subsection{Semantic Cross Attention}
Let's first explain the mechanism that will allow giving each feature map information from a semantically restricted set of latents. Let's call $Y\in\mathbb{R}^{m\times d}$ a set of m latents of dimension $d$ and $s$ the number of different semantic labels. Each semantic label will get attributed  $k$ latents vectors, such as $m=k\times s$. Similarly, $X\in\mathbb{R}^{H\times W\times C}$ is a given image or feature map of an encoded image and $S_{2D}\in\{0;1\}^{H\times W \times s}$ the associated segmentation mask.

To perform the attention computation, the image is flattened according to the spatial dimensions, yielding $X_{flat}\in\mathbb{R}^{n\times C}$ where $n = H\times W$.
The segmentation map is duplicated making $k$ copies of each channel dimension, making sure that each of the latents have its respective segmentation map. This operation gives $S\in\{0;1\}^{n \times m}$.

Now, let's have $W_{Q}\in\mathbb{R}^{n\times d_{in}}$, $W_{Q}\in\mathbb{R}^{m\times d_{in}}$ and $W_{K}\in\mathbb{R}^{m\times d_{in}}$, allowing to compute queries, keys and values ($Q = W_QX_{flatten}$, $K = W_KY$ and $V = W_VY$)
The idea to compute the masked attention is to destroy any attention values where the pixel from a semantic region is not attending the latents from that semantic region. These attention values requiring masking are filled with $-10^9$ before the softmax the values. Let's denote by $\sigma(.)$ the softmax operation. The following equation shows how to compute the semantic cross-attention:
\begin{equation}
    SCA(X_{flat},Y, S) = \sigma\left(\frac{QK^T\odot S -10^9 \left(1-S\right)}{\sqrt{d_{in}}}\right)V
\end{equation}

Now, deriving $SCA(Y,X_{flat}, S)$ is straightforward. The idea is to semantically mask attention values to enforce latents to attend semantically corresponding pixels. Having $W_{Q}\in\mathbb{R}^{m\times d_{in}}$, $W_{Q}\in\mathbb{R}^{n\times d_{in}}$ and $W_{K}\in\mathbb{R}^{n\times d_{in}}$ allowing to compute queries, keys and values ($Q = W_QY$, $K = W_KX_{flat}$ and $V = W_VX_{flat}$)

The computation of SCA for pixels to latents is the following:
\begin{equation}
    SCA(Y,X_{flat},S) = \sigma\left(\frac{QK^T\odot S^T -10^9 \left(1-S^T\right)}{\sqrt{d_{in}}}\right)V
\end{equation}


\subsection{The Encoder}

\input{sections/encoder}

\subsection{The Generator}

\input{sections/generator}

\subsection{Training details}
We train the system with a combination of GAN and reconstruction loss. For the GAN loss, we use Hinge GAN loss \cite{lim2017geometric}. If we denote by D the discriminator, G the generator, E the Encoder, $X$ the images and $S$ the associated segmentation masks we have the following GAN loss:
\begin{equation}
    \begin{split}
        &\mathcal{L}_{D,GAN} = \mathbb{E}\left[ max(0,1-D(X,S))\right]\\ &+\mathbb{E}\left[ max(0,D(G(E(X,S),S),S)+1)\right]
    \end{split}
\end{equation}

\begin{equation}
    \mathcal{L}_{G,GAN} = \mathbb{E}\left[D(G(E(X,S),S),S)\right]
\end{equation}

For the discriminator, we are going to use the PatchGAN discriminator \cite{isola2018imagetoimage}, following the works of Pix2Pix \cite{isola2018imagetoimage}, Pix2PixHD\cite{wang2018pix2pixHD}, SPADE\cite{park2019semantic} and SEAN\cite{Zhu_2020}. The idea is that the PatchGAN discriminator discriminates for patches of the given image instead of discriminating the global image. This allows to focus the GAN objective on the high-frequency content, leaving the low frequency content to the reconstruction loss. We concatenate both the image and the segmentation mask before using the discriminator.

Finally, for the reconstruction loss, we keep the perceptual loss from SEAN. The perceptual loss uses a pretrained VGG network, and we try to make the intermediate feature maps between the input and the reconstructed input as close as possible. This gives the following loss:
\begin{equation}
     \mathcal{L}_{VGG} = \mathbb{E}\left[\sum_{i=1}^L\lVert F_i(X) - F_i(G(E(X,S))) \rVert_1 \right]
\end{equation}
with L the number of VGG hidden layers and $F_i$ the $i^{th}$ layer feature map of the VGG feature map.

However, we do not keep the Feature Matching loss. We observe that when having more difficult datasets, the Feature Matching loss fails to train the GAN and collapse training. We replace it by the $\mathcal{L}_1$ loss.
\begin{equation}
    \mathcal{L}_1=\mathbb{E}[\lVert X-G(E(X,S))\rVert_1]
\end{equation}

Finally, we have the following loss for the generator and the discriminator:
\begin{equation}
    \mathcal{L}_{G} =  \mathcal{L}_{G,GAN} + \lambda_{perceptual}\mathcal{L}_{VGG} + \lambda_{1}\mathcal{L}_{1}
\end{equation}
with $\lambda_{perceptual}$ and $\lambda_{1}$ hyperparameters. We will take $\lambda_{perceptual}=\lambda_{1}=10$. We observe that using smaller values could lead to training collapse.
\begin{equation}
    \mathcal{L}_{D} = \mathcal{L}_{D,GAN}
\end{equation}

==> sections/relatedwork_original.tex <==
\noindent \textbf{Image Generation with GANs.} 
Generative Adversarial Networks \cite{goodfellow2014generative} have proven to be useful at generating images from a given distribution. Having a generator and a discriminator competing to fool each other allows detecting errors in the generation and progressively improving them. Multiple improvements \cite{lapgan, dcgan, karras2018progressive} have allowed the generation of high-quality images. A major improvement was StyleGAN \cite{karras2019stylebased, karras2020analyzing, Karras2021} which propose a novel normalization technique that allowed to modulate the feature map at each resolution according to a given style vector. Recently, GANsformer \cite{hudson2021generative} has proposed to improve this modulation by leveraging multiple style codes using a cross attention mechanism between a set of style vectors and the feature maps. This paper has shown the emergence of semantic structure with the specialization of the latents according to different semantically meaningful objects.

\paragraph{Image to Image synthesis with GANs} Naive unconditional GANs allows for minimal control over the output of the generator. To allow for more flexible systems, Pix2Pix \cite{isola2018imagetoimage, wang2018pix2pixHD} propose to train the generator coupled to an encoder. This allows to condition the generation according to an input image. Pix2Pix allows controlling the output with multiple modalities such as sketches, keypoints, or segmentation maps. One of the drawbacks of Pix2Pix is the need for aligned pairs of data. This can be hard to collect in some cases (Drawings for example), or even impossible in some cases. That's why CycleGAN \cite{zhu2020unpaired} propose a method to work with unpaired data. The idea is to enforce a cycle consistency between the domains from which we want to translate to. For semantic masks, acquiring paired data is not as hard as other modalities thanks to segmentation networks that can be used to label data. To perform semantic masks to image translation, SPADE \cite{park2019semantic} improves upon Pix2Pix. Indeed, the authors observed that when providing the semantic information only at the input of the generator, the segmentation map can get washed up by the normalization layer. Therefore, in SPADE, the semantic information is provided at all layers of the generator, having the semantic information modulate the feature maps. One of the drawbacks of SPADE is that the style is only controlled at the input of the generator. As StyleGAN has showed, it is highly beneficial to control the style at each layer of the generator network. Moreover, there is only a single style vector for all semantic labels. SPADE is very good to generate images from a semantic mask but lacks in performance when trying to reconstruct images conditioned on semantic masks. Image reconstruction is an important task if we want to be able to edit such image afterwards.  SEAN \cite{Zhu_2020} address these issues by modulating at each layer by both semantic information and style vectors. SEAN introduces one style vector per semantic region to enable finer semantic editing. To do so, the authors encode the desired image and then average pool the pixels according to a semantic map into a single style vector per region.

\paragraph{Attention in Computer Vision} Transformers have had great success in fields such as NLP \cite{devlin2019bert, radford2018improving, radford2019language, brown2020language}. However, transformers suffer from a quadratic complexity problem. This makes it harder to be used in computer vision, since a pixel cannot be considered as a single token. Some works have proposed to linearize the attention mechanism\cite{wang2020linformer, kitaev2020reformer, choromanski2021rethinking}. However, these methods are not widely used in computer vision yet. The trick that manages to make transformers work for computer vision is to subdivide the image into non-overlapping patches that are encoded using a linear mapping. This idea was introduced in ViT \cite{dosovitskiy2021image}. However, by having images treated as patches, we can lose the information inside the patches. Perceiver \cite{jaegle2021perceiver, jaegle2021perceiverio} proposed to solve the quadratic complexity problem by replacing self attention by cross attention. The idea is to attend the image pixels to a set of learned tokens that are going to retrieve information from the tokens. In GANs, attention was first used in the works of SAGAN \cite{zhang2019selfattention}, where self-attention was performed on the low-resolutions layers of the generator to avoid the quadratic complexity problem. Recently, VQ-GAN \cite{esser2021taming} learns a fixed codebook that is then manipulated thanks to a transformer to select the relevant codes to generate the desired image. TransGAN\cite{jiang2021transgan} has replaced both the generator and the discriminator by transformer networks.

\paragraph{Human Pose Transfer}
A few works have performed human pose transfer using keypoints. For example, \cite{ma2017pose}, use a Pix2Pix like network to perform keypoints to image translation, using first a coarser output that is then refined by a higher resolution generator. \cite{zhu2019progressive} propose to progressively incorporate the keypoint knowledge in the image subnetwork. Similarly, \cite{tang2020xinggan} propose to encode with two subnetworks pose and image and then merge the representation with a co-attention module. Another method that uses Keypoints is \cite{li2020pona}, which propose to use a long-range attention module to account for global interactions. All these methods relies on keypoints and therefore only have a coarse representation of the body. That's why we think it's preferable to work with semantic masks. Such approach has also been followed by works such as \cite{han2019clothflow, dong2018soft, zhang2020human}. PISA \cite{zhang2021pise} use this segmentation masks with a SEAN \cite{Zhu_2020} like network to perform pose transfer. However, all this previous works focus on pose transfer, which does not alter the background. Our goal is to perform subject transfer where we need to handle the background. Moreover, previous works work use datasets which quite simple backgrounds. On videos, \cite{chan2019everybody} propose to overfit a GAN to the whole video, therefore regenerating the background. However, this only works for static backgrounds and needs a lot of data and compute for a single pose transfer. A solution was proposed by \cite{wang2018fewshotvid2vid} that propose to learn a hyper network to adapt the weights of the generator, but this technique still ties the subject to the background not allowing to perform subject transfer.
